Generative Language Models and Automated Influence Operations: Emerging Threats and Potential Mitigations

Generative language models have improved drastically, and can now produce realistic text outputs that are difficult to distinguish from human-written content. For malicious actors, these language models bring the promise of automating the creation of convincing and misleading text for use in influence operations. This report assesses how language models might change influence operations in the future, and what steps can be taken to mitigate this threat. We lay out possible changes to the actors, behaviors, and content of online influence operations, and provide a framework for stages of the language model-to-influence operations pipeline that mitigations could target (model construction, model access, content dissemination, and belief formation). While no reasonable mitigation can be expected to fully prevent the threat of AI-enabled influence operations, a combination of multiple mitigations may make an important difference.

==> autogen_table.tex <==
% Pasting the auto generated version of table 2 here for preservation
% Be careful that you copy all of this (30 lines) if using

\begin{table}[ht]
\begin{tabular}{lll}
\hline
\multicolumn{1}{|l|}{{\color[HTML]{000000} \textbf{\begin{tabular}[M{0.3\linewidth}]{@{}l@{}}What Propagandists \\ Require\end{tabular}}}}                                               & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}l@{}}Stage of \\ Intervention\end{tabular}}}}                        & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{Illustrative Mitigations}}}                                                                                                                                                                                                                                                                                                                               \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}1. Language Models \\ Capable of Producing \\ Realistic Text\end{tabular}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Model Design and \\ Construction\end{tabular}}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}-AI Developers Build Models That Are \\   More Fact-Sensitive\\ -Developers Spread Radioactive Data to \\   Make Generative Models Detectable\\ -Governments Impose Restrictions on \\   Data Collection\\ -Governments Impose Access Controls \\   on AI Hardware\end{tabular}}}                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                                                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                                                                                                                                                                                                                                                                                        \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                                                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }}                                                                                                                                                                                                                                                                                                                                        \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}2. Reliable Access to \\ Such Models\end{tabular}}}}       & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Model Access}}}                                           & \multicolumn{1}{l|}{\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}-AI Providers Impose Stricter Usage \\   Restrictions on Language Models\\ -AI Providers Develop New Norms Around \\   Model Release\\ -AI Providers Close Security Vulnerabilities\end{tabular}}}}                                                                                           \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}3. Infrastructure to \\ Distribute the \\ Generated Content\end{tabular}}}  & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Content \\ Dissemination\end{tabular}}}         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}-Platforms and AI Providers Coordinate to \\   Identify AI Content\\ -Platforms Require “Proof of Personhood” \\   to Post\\ -Entities That Rely on Public Input Take \\   Steps to Reduce Their Exposure to \\   Misleading AI Content\\ -Digital Provenance Standards Are Widely \\   Adopted\end{tabular}}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}4. Susceptible Target\\ Audience\end{tabular}}}                             & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Belief Formation}}                                                         & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}-Institutions Engage In Media Literacy Campaigns\\ -Developers Provide Consumer Focused AI Tools\end{tabular}}}                                                                                                                                                                                                                                          \\ \hline
\rowcolor[HTML]{FFFFFF} 
                                                                                                                                                                          & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}}                                                                                                 &                                                                                                                                                                                                                                                                                                                                                                                                             \\
\rowcolor[HTML]{FFFFFF} 
                                                                                                                                                                          & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}}                                                                                                 & \cellcolor[HTML]{FFFFFF}                                                                                                                                                                                                                                                                                                                                                                                    \\
                                                                                                                                                                          & \multicolumn{1}{c}{}                                                                                                                         & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}}                                                                                                                                                                                                                                                                                                                                                                  \\
                                                                                                                                                                          & \multicolumn{1}{c}{}                                                                                                                         &                                                                                                                                                                                                                                                                                                                                                                                                             \\
                                                                                                                                                                          & \multicolumn{1}{c}{}                                                                                                                         &                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
\end{tabular}
\caption{}
\label{tab:propaganda}
\end{table}
